Non-Perturbative Simulations of Quantum Field Theories using Complex Langevin Dynamics

Non-perturbative formulations of field theories are essential to capture intriguing physical phenomena, including confinement in QCD, spontaneous supersymmetry breaking, and dynamical compactification in superstrings. Lattice regularization provides a robust framework to study these non-perturbative features through Euclidean path integrals. Conventionally, path integrals are numerically evaluated using Monte Carlo methods, where the Boltzmann factor is interpreted as a probability weight. However, complex actions in various physical systems render the Boltzmann factor complex, leading to the sign problem. The complex Langevin method overcomes the sign problem and can be used to evaluate complex integrals. This thesis employs the complex Langevin method to investigate various non-perturbative aspects of field-theoretic systems with complex actions. We probe the possibility of spontaneous supersymmetry breaking in the simplest realizations of supersymmetric field theories. These systems generally have complex actions arising from a complex determinant of the fermion operator. We studied various interesting classes of complex potentials, including those exhibiting PT-symmetry. Another exciting aspect explored is the dynamical compactification of extra dimensions in superstring theory. The IKKT matrix model, in the large-N limit, is a conjectured formulation for the 10D type IIB string theory. We employ the complex Langevin method to investigate the Euclidean version of this matrix model, which has an inherent complex Pfaffian, to probe the spontaneous breaking of SO(10) symmetry. The investigations performed in this thesis suggest that the complex Langevin method can successfully simulate non-perturbative aspects of quantum field theories by taming the associated sign problem.

==> bibliography.tex <==
\begin{thebibliography}{100}

\bibitem{Witten:1981nf}
E.~Witten, \emph{{Dynamical Breaking of Supersymmetry}},
\href{https://doi.org/10.1016/0550-3213(81)90006-7}{\emph{Nucl. Phys.}
	{\bfseries B188} (1981) 513}.

\bibitem{Witten:1982df}
E.~Witten, \emph{{Constraints on Supersymmetry Breaking}},
\href{https://doi.org/10.1016/0550-3213(82)90071-2}{\emph{Nucl. Phys. B}
	{\bfseries 202} (1982) 253}.


\bibitem{Klauder:1983nn}
J.~R. Klauder, \emph{Stochastic Quantization},
\href{http://dx.doi.org/10.1007/978-3-7091-7651-1_8}{{\em Acta Phys. Austriaca
		Suppl.} {\bfseries 25} (1983) 251--281}.
%%CITATION = APAUA,25,251;%%.

\bibitem{Klauder:1983zm}
J.~R. Klauder, \emph{A Langevin Approach to Fermion and Quantum Spin Correlation
	Functions},
\href{http://dx.doi.org/10.1088/0305-4470/16/10/001}{{\em J. Phys.} {\bfseries
		A16} (1983) L317}.
%%CITATION = JPAGA,A16,L317;%%.

\bibitem{Klauder:1983sp}
J.~R. Klauder, \emph{Coherent State Langevin Equations for Canonical Quantum
	Systems With Applications to the Quantized Hall Effect},
\href{http://dx.doi.org/10.1103/PhysRevA.29.2036}{{\em Phys. Rev.} {\bfseries
		A29} (1984) 2036--2047}.
%%CITATION = PHRVA,A29,2036;%%.

\bibitem{Parisi:1984cs}
G.~Parisi, \emph{On Complex Probabilities},
\href{http://dx.doi.org/10.1016/0370-2693(83)90525-7}{{\em Phys. Lett.}
	{\bfseries 131B} (1983) 393--395}.
%%CITATION = PHLTA,131B,393;%%.

\bibitem{Cristoforetti:2012su}
{\bfseries AuroraScience} Collaboration, M.~Cristoforetti, F.~Di~Renzo, and
L.~Scorzato, \emph{New approach to the sign problem in quantum field theories:
	High density QCD on a Lefschetz thimble},
\href{http://dx.doi.org/10.1103/PhysRevD.86.074506}{{\em Phys. Rev.}
	{\bfseries D86} (2012) 074506},
\href{http://arxiv.org/abs/1205.3996}{{\ttfamily arXiv:1205.3996 [hep-lat]}}.
%%CITATION = ARXIV:1205.3996;%%.

\bibitem{Fujii:2013sra}
H.~Fujii, D.~Honda, M.~Kato, Y.~Kikukawa, S.~Komatsu, and T.~Sano, \emph{Hybrid
	Monte Carlo on Lefschetz thimbles - A study of the residual sign problem},
\href{http://dx.doi.org/10.1007/JHEP10(2013)147}{{\em JHEP} {\bfseries 10}
	(2013) 147},
\href{http://arxiv.org/abs/1309.4371}{{\ttfamily arXiv:1309.4371 [hep-lat]}}.
%%CITATION = ARXIV:1309.4371;%%.

\bibitem{DiRenzo:2015foa}
F.~Di~Renzo and G.~Eruzzi, \emph{Thimble regularization at work: from toy models
	to chiral random matrix theories},
\href{http://dx.doi.org/10.1103/PhysRevD.92.085030}{{\em Phys. Rev.}
	{\bfseries D92} no.~8, (2015) 085030},
\href{http://arxiv.org/abs/1507.03858}{{\ttfamily arXiv:1507.03858 [hep-lat]}}.
%%CITATION = ARXIV:1507.03858;%%.

\bibitem{Tanizaki:2015rda}
Y.~Tanizaki, Y.~Hidaka, and T.~Hayata, \emph{Lefschetz-thimble analysis of the
	sign problem in one-site fermion model},
\href{http://dx.doi.org/10.1088/1367-2630/18/3/033002}{{\em New J. Phys.}
	{\bfseries 18} no.~3, (2016) 033002},
\href{http://arxiv.org/abs/1509.07146}{{\ttfamily arXiv:1509.07146 [hep-th]}}.
%%CITATION = ARXIV:1509.07146;%%.

\bibitem{Fujii:2015vha}
H.~Fujii, S.~Kamata, and Y.~Kikukawa, \emph{Monte Carlo study of Lefschetz thimble
	structure in one-dimensional Thirring model at finite density},
\href{http://dx.doi.org/10.1007/JHEP12(2015)125,
	10.1007/JHEP09(2016)172}{{\em JHEP} {\bfseries 12} (2015) 125},
\href{http://arxiv.org/abs/1509.09141}{{\ttfamily arXiv:1509.09141
		[hep-lat]}}.
[Erratum: JHEP09,172(2016)].
%%CITATION = ARXIV:1509.09141;%%.

\bibitem{Alexandru:2015xva}
A.~Alexandru, G.~Basar, and P.~Bedaque, \emph{Monte Carlo algorithm for simulating
	fermions on Lefschetz thimbles},
\href{http://dx.doi.org/10.1103/PhysRevD.93.014504}{{\em Phys. Rev.}
	{\bfseries D93} no.~1, (2016) 014504},
\href{http://arxiv.org/abs/1510.03258}{{\ttfamily arXiv:1510.03258 [hep-lat]}}.
%%CITATION = ARXIV:1510.03258;%%.

\bibitem{Damgaard:1987rr}
P.~H. Damgaard and H.~Huffel, \emph{Stochastic Quantization},
\href{http://dx.doi.org/10.1016/0370-1573(87)90144-X}{{\em Phys. Rept.}
	{\bfseries 152} (1987) 227}.
%%CITATION = PRPLC,152,227;%%.


\bibitem{deForcrand:2002hgr}
P.~de~Forcrand and O.~Philipsen, \emph{{The QCD phase diagram for small
		densities from imaginary chemical potential}},
\href{https://doi.org/10.1016/S0550-3213(02)00626-0}{\emph{Nucl. Phys. B}
	{\bfseries 642} (2002) 290}
[\href{https://arxiv.org/abs/hep-lat/0205016}{{\ttfamily hep-lat/0205016}}].


\bibitem{Aarts:2009dg}
G.~Aarts, F.A.~James, E.~Seiler and I.-O.~Stamatescu, \emph{{Adaptive stepsize
		and instabilities in complex Langevin dynamics}},
\href{https://doi.org/10.1016/j.physletb.2010.03.012}{\emph{Phys. Lett. B}
	{\bfseries 687} (2010) 154}
[\href{https://arxiv.org/abs/0912.0617}{{\ttfamily 0912.0617}}].

\bibitem{Berger:2019odf}
C.~E. Berger, L.~Rammelmuller, A.~C. Loheac, F.~Ehmann, J.~Braun, and J.~E.
Drut, \emph{Complex Langevin and other approaches to the sign problem in quantum
	many-body physics},
\href{http://arxiv.org/abs/1907.10183}{{\ttfamily arXiv:1907.10183
		[cond-mat.quant-gas]}}.
%%CITATION = ARXIV:1907.10183;%%.

\bibitem{Berges:2005yt}
J.~Berges and I.~O. Stamatescu, \emph{Simulating nonequilibrium quantum fields
	with stochastic quantization techniques},
\href{http://dx.doi.org/10.1103/PhysRevLett.95.202003}{{\em Phys. Rev. Lett.}
	{\bfseries 95} (2005) 202003},
\href{http://arxiv.org/abs/hep-lat/0508030}{{\ttfamily arXiv:hep-lat/0508030
		[hep-lat]}}.
%%CITATION = HEP-LAT/0508030;%%.

\bibitem{Berges:2006xc}
J.~Berges, S.~Borsanyi, D.~Sexty, and I.~O. Stamatescu, \emph{Lattice simulations
	of real-time quantum fields},
\href{http://dx.doi.org/10.1103/PhysRevD.75.045007}{{\em Phys. Rev.}
	{\bfseries D75} (2007) 045007},
\href{http://arxiv.org/abs/hep-lat/0609058}{{\ttfamily arXiv:hep-lat/0609058
		[hep-lat]}}.
%%CITATION = HEP-LAT/0609058;%%.

\bibitem{Berges:2007nr}
J.~Berges and D.~Sexty, \emph{Real-time gauge theory simulations from stochastic
	quantization with optimized updating},
\href{http://dx.doi.org/10.1016/j.nuclphysb.2008.01.018}{{\em Nucl. Phys.}
	{\bfseries B799} (2008) 306--329},
\href{http://arxiv.org/abs/0708.0779}{{\ttfamily arXiv:0708.0779 [hep-lat]}}.
%%CITATION = ARXIV:0708.0779;%%.

\bibitem{Bloch:2017sex}
J.~Bloch, J.~Glesaaen, J.~J.~M. Verbaarschot, and S.~Zafeiropoulos, \emph{Complex
	Langevin Simulation of a Random Matrix Model at Nonzero Chemical
	Potential}, \href{http://dx.doi.org/10.1007/JHEP03(2018)015}{{\em JHEP}
	{\bfseries 03} (2018) 015},
\href{http://arxiv.org/abs/1712.07514}{{\ttfamily arXiv:1712.07514 [hep-lat]}}.
%%CITATION = ARXIV:1712.07514;%%.

\bibitem{Aarts:2008rr}
G.~Aarts and I.-O. Stamatescu, \emph{Stochastic quantization at finite chemical
	potential}, \href{http://dx.doi.org/10.1088/1126-6708/2008/09/018}{{\em
		JHEP} {\bfseries 09} (2008) 018},
\href{http://arxiv.org/abs/0807.1597}{{\ttfamily arXiv:0807.1597 [hep-lat]}}.
%%CITATION = ARXIV:0807.1597;%%.

\bibitem{Pehlevan:2007eq}
C.~Pehlevan and G.~Guralnik, \emph{Complex Langevin Equations and Schwinger-Dyson
	Equations}, \href{http://dx.doi.org/10.1016/j.nuclphysb.2008.11.034}{{\em
		Nucl. Phys.} {\bfseries B811} (2009) 519--536},
\href{http://arxiv.org/abs/0710.3756}{{\ttfamily arXiv:0710.3756 [hep-th]}}.
%%CITATION = ARXIV:0710.3756;%%.

\bibitem{Aarts:2008wh}
G.~Aarts, \emph{Can stochastic quantization evade the sign problem? The
	relativistic Bose gas at finite chemical potential},
\href{http://dx.doi.org/10.1103/PhysRevLett.102.131601}{{\em Phys. Rev.
		Lett.} {\bfseries 102} (2009) 131601},
\href{http://arxiv.org/abs/0810.2089}{{\ttfamily arXiv:0810.2089 [hep-lat]}}.
%%CITATION = ARXIV:0810.2089;%%.

\bibitem{Aarts:2009hn}
G.~Aarts, \emph{Complex Langevin dynamics at finite chemical potential: Mean field
	analysis in the relativistic Bose gas},
\href{http://dx.doi.org/10.1088/1126-6708/2009/05/052}{{\em JHEP} {\bfseries
		05} (2009) 052},
\href{http://arxiv.org/abs/0902.4686}{{\ttfamily arXiv:0902.4686 [hep-lat]}}.
%%CITATION = ARXIV:0902.4686;%%.

\bibitem{Aarts:2010gr}
G.~Aarts and K.~Splittorff, \emph{Degenerate distributions in complex Langevin
	dynamics: one-dimensional QCD at finite chemical potential},
\href{http://dx.doi.org/10.1007/JHEP08(2010)017}{{\em JHEP} {\bfseries 08}
	(2010) 017},
\href{http://arxiv.org/abs/1006.0332}{{\ttfamily arXiv:1006.0332 [hep-lat]}}.
%%CITATION = ARXIV:1006.0332;%%.

\bibitem{Aarts:2011zn}
G.~Aarts and F.~A. James, \emph{Complex Langevin dynamics in the SU(3) spin model
	at nonzero chemical potential revisited},
\href{http://dx.doi.org/10.1007/JHEP01(2012)118}{{\em JHEP} {\bfseries 01}
	(2012) 118},
\href{http://arxiv.org/abs/1112.4655}{{\ttfamily arXiv:1112.4655 [hep-lat]}}.
%%CITATION = ARXIV:1112.4655;%%.

\bibitem{Ito:2016efb}
Y.~Ito and J.~Nishimura, \emph{The complex Langevin analysis of spontaneous
	symmetry breaking induced by complex fermion determinant},
\href{http://dx.doi.org/10.1007/JHEP12(2016)009}{{\em JHEP} {\bfseries 12}
	(2016) 009},
\href{http://arxiv.org/abs/1609.04501}{{\ttfamily arXiv:1609.04501 [hep-lat]}}.
%%CITATION = ARXIV:1609.04501;%%.

\bibitem{Ito:2016hlj}
Y.~Ito and J.~Nishimura, \emph{Spontaneous symmetry breaking induced by complex
	fermion determinant --- yet another success of the complex Langevin
	method}, \href{http://dx.doi.org/10.22323/1.256.0065}{{\em PoS} {\bfseries
		LATTICE2016} (2016) 065},
\href{http://arxiv.org/abs/1612.00598}{{\ttfamily arXiv:1612.00598 [hep-lat]}}.
%%CITATION = ARXIV:1612.00598;%%.

\bibitem{Anagnostopoulos:2017gos}
K.~N. Anagnostopoulos, T.~Azuma, Y.~Ito, J.~Nishimura, and S.~K. Papadoudis,
\emph{Complex Langevin analysis of the spontaneous symmetry breaking in
	dimensionally reduced super Yang-Mills models},
\href{http://dx.doi.org/10.1007/JHEP02(2018)151}{{\em JHEP} {\bfseries 02}
	(2018) 151},
\href{http://arxiv.org/abs/1712.07562}{{\ttfamily arXiv:1712.07562 [hep-lat]}}.
%%CITATION = ARXIV:1712.07562;%%.

\bibitem{Basu:2018dtm}
P.~Basu, K.~Jaswin, and A.~Joseph, \emph{Complex Langevin Dynamics in Large $N$
	Unitary Matrix Models},
\href{http://dx.doi.org/10.1103/PhysRevD.98.034501}{{\em Phys. Rev.}
	{\bfseries D98} no.~3, (2018) 034501},
\href{http://arxiv.org/abs/1802.10381}{{\ttfamily arXiv:1802.10381 [hep-th]}}.
%%CITATION = ARXIV:1802.10381;%%.

\bibitem{Gross:1980he}
D.~J. Gross and E.~Witten, \emph{Possible Third Order Phase Transition in the
	Large N Lattice Gauge Theory},
\href{http://dx.doi.org/10.1103/PhysRevD.21.446}{{\em Phys. Rev.} {\bfseries
		D21} (1980) 446--453}.


\bibitem{Wadia:1980cp}
S.~R. Wadia, \emph{$N$ = Infinity Phase Transition in a Class of Exactly Soluble
	Model Lattice Gauge Theories},
\href{http://dx.doi.org/10.1016/0370-2693(80)90353-6}{{\em Phys. Lett.}
	{\bfseries 93B} (1980) 403--410}.
%%CITATION = PHLTA,93B,403;%%.

\bibitem{Aarts:2009uq}
G.~Aarts, E.~Seiler, and I.-O. Stamatescu, \emph{The Complex Langevin method: When
	can it be trusted?},
\href{http://dx.doi.org/10.1103/PhysRevD.81.054508}{{\em Phys. Rev.}
	{\bfseries D81} (2010) 054508},
\href{http://arxiv.org/abs/0912.3360}{{\ttfamily arXiv:0912.3360 [hep-lat]}}.
%%CITATION = ARXIV:0912.3360;%%.

\bibitem{Aarts:2011ax}
G.~Aarts, F.~A. James, E.~Seiler, and I.-O. Stamatescu, \emph{Complex Langevin:
	Etiology and Diagnostics of its Main Problem},
\href{http://dx.doi.org/10.1140/epjc/s10052-011-1756-5}{{\em Eur. Phys. J.}
	{\bfseries C71} (2011) 1756},
\href{http://arxiv.org/abs/1101.3270}{{\ttfamily arXiv:1101.3270 [hep-lat]}}.
%%CITATION = ARXIV:1101.3270;%%.

\bibitem{Nagata:2015uga}
K.~Nagata, J.~Nishimura, and S.~Shimasaki, \emph{Justification of the complex
	Langevin method with the gauge cooling procedure},
\href{http://dx.doi.org/10.1093/ptep/ptv173}{{\em PTEP} {\bfseries 2016}
	no.~1, (2016) 013B01},
\href{http://arxiv.org/abs/1508.02377}{{\ttfamily arXiv:1508.02377 [hep-lat]}}.
%%CITATION = ARXIV:1508.02377;%%.

\bibitem{Klauder:1985kq}
J.~R. Klauder and W.~P. Petersen, \emph{Numerical Integration of Multiplicative-Noise Stochastic Differential Equations},
{\em SIAM J. Num. Anal.} {\bfseries 22} (1985) 1153--1166.
%%CITATION = PRINT-85-0297 (BTL);%%.

\bibitem{Klauder:1985ks}
J.~R. Klauder and W.~P. Petersen, \emph{Spectrum of certain non-self-adjoint operators and solutions of Langevin equations with complex drift},
{\em J. Stat. Phys.} {\bfseries 39} (1985) 53--72.
%%CITATION = PRINT-85-0295 (BTL);%%.

\bibitem{Gausterer:1986gk}
H.~Gausterer and J.~R. Klauder, \emph{Complex Langevin Equations and Their
	Applications to Quantum Statistical and Lattice Field Models},
\href{http://dx.doi.org/10.1103/PhysRevD.33.3678}{{\em Phys. Rev.} {\bfseries
		D33} (1986) 3678}.
%%CITATION = PHRVA,D33,3678;%%.

\bibitem{Bender:1997ps}
C.~M. Bender and K.~A. Milton, \emph{Model of supersymmetric quantum field theory
	with broken parity symmetry},
\href{http://dx.doi.org/10.1103/PhysRevD.57.3595}{{\em Phys. Rev.} {\bfseries
		D57} (1998) 3595--3608},
\href{http://arxiv.org/abs/hep-th/9710076}{{\ttfamily arXiv:hep-th/9710076
		[hep-th]}}.
%%CITATION = HEP-TH/9710076;%%.

\bibitem{ToAppear:2019}
A.~Joseph and A.~Kumar, \emph{In preparation},.

\bibitem{Bender:1999ek}
C.~M. Bender, K.~A. Milton, and V.~M. Savage, \emph{Solution of Schwinger-Dyson
	equations for PT symmetric quantum field theory},
\href{http://dx.doi.org/10.1103/PhysRevD.62.085001}{{\em Phys. Rev.}
	{\bfseries D62} (2000) 085001},
\href{http://arxiv.org/abs/hep-th/9907045}{{\ttfamily arXiv:hep-th/9907045
		[hep-th]}}.
%%CITATION = HEP-TH/9907045;%%.

\bibitem{Kuroki:2009yg}
T.~Kuroki and F.~Sugino, \emph{Spontaneous supersymmetry breaking in large-N
	matrix models with slowly varying potential},
\href{http://dx.doi.org/10.1016/j.nuclphysb.2009.12.021}{{\em Nucl. Phys.}
	{\bfseries B830} (2010) 434--473},
\href{http://arxiv.org/abs/0909.3952}{{\ttfamily arXiv:0909.3952 [hep-th]}}.
%%CITATION = ARXIV:0909.3952;%%.

\bibitem{Kuroki:2010au}
T.~Kuroki and F.~Sugino, \emph{Spontaneous supersymmetry breaking in matrix models
	from the viewpoints of localization and Nicolai mapping},
\href{http://dx.doi.org/10.1016/j.nuclphysb.2010.11.015}{{\em Nucl. Phys.}
	{\bfseries B844} (2011) 409--449},
\href{http://arxiv.org/abs/1009.6097}{{\ttfamily arXiv:1009.6097 [hep-th]}}.
%%CITATION = ARXIV:1009.6097;%%.

\bibitem{Aarts:2013uza}
G.~Aarts, P.~Giudice, and E.~Seiler, \emph{Localised distributions and criteria
	for correctness in complex Langevin dynamics},
\href{http://dx.doi.org/10.1016/j.aop.2013.06.019}{{\em Annals Phys.}
	{\bfseries 337} (2013) 238--260},
\href{http://arxiv.org/abs/1306.3075}{{\ttfamily arXiv:1306.3075 [hep-lat]}}.
%%CITATION = ARXIV:1306.3075;%%.

\bibitem{Nagata:2016vkn}
K.~Nagata, J.~Nishimura, and S.~Shimasaki, \emph{Argument for justification of the
	complex Langevin method and the condition for correct convergence},
\href{http://dx.doi.org/10.1103/PhysRevD.94.114515}{{\em Phys. Rev.}
	{\bfseries D94} no.~11, (2016) 114515},
\href{http://arxiv.org/abs/1606.07627}{{\ttfamily arXiv:1606.07627 [hep-lat]}}.
%%CITATION = ARXIV:1606.07627;%%.

\bibitem{Nagata:2018net}
K.~Nagata, J.~Nishimura, and S.~Shimasaki, \emph{Testing the criterion for correct
	convergence in the complex Langevin method},
\href{http://dx.doi.org/10.1007/JHEP05(2018)004}{{\em JHEP} {\bfseries 05}
	(2018) 004},
\href{http://arxiv.org/abs/1802.01876}{{\ttfamily arXiv:1802.01876 [hep-lat]}}.
%%CITATION = ARXIV:1802.01876;%%.


%%%%
%WZ model

%\cite{Bender:1997ps}
\bibitem{Bender:1997ps}
C.~M.~Bender and K.~A.~Milton,
\emph{Model of supersymmetric quantum field theory with broken parity symmetry,}
Phys. Rev. D \textbf{57} (1998), 3595-3608
doi:10.1103/PhysRevD.57.3595
[arXiv:hep-th/9710076 [hep-th]].
%49 citations counted in INSPIRE as of 07 Aug 2021

%\cite{Bender:1998gh}
\bibitem{Bender:1998gh}
C.~M.~Bender, S.~Boettcher and P.~Meisinger,
\emph{PT symmetric quantum mechanics,}
J. Math. Phys. \textbf{40}, 2201-2229 (1999)
doi:10.1063/1.532860
[arXiv:quant-ph/9809072 [quant-ph]].
%473 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Witten:1981nf}
\bibitem{Witten:1981nf}
E.~Witten,
\emph{Dynamical breaking of supersymmetry,}
Nucl. Phys. B \textbf{188}, 513 (1981)
doi:10.1016/0550-3213(81)90006-7
%3338 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Witten:1982df}
\bibitem{Witten:1982df}
E.~Witten,
\emph{Constraints on supersymmetry breaking,}
Nucl. Phys. B \textbf{202}, 253 (1982)
doi:10.1016/0550-3213(82)90071-2
%1789 citations counted in INSPIRE as of 26 Jan 2022

%\cite{De:2005ny}
\bibitem{De:2005ny}
A.~K.~De, A.~Harindranath, J.~Maiti and T.~Sinha,
\emph{Investigations in 1+1 dimensional lattice $\phi^4$ theory,}
Phys. Rev. D \textbf{72}, 094503 (2005)
doi:10.1103/PhysRevD.72.094503
[arXiv:hep-lat/0506002 [hep-lat]].
%8 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Schaich:2009jk}
\bibitem{Schaich:2009jk}
D.~Schaich and W.~Loinaz,
\emph{An Improved lattice measurement of the critical coupling in $\phi_2^4$ theory,}
Phys. Rev. D \textbf{79}, 056008 (2009)
doi:10.1103/PhysRevD.79.056008
[arXiv:0902.0045 [hep-lat]].
%42 citations counted in INSPIRE as of 26 Jan 2022	

%\cite{Wozar:2011gu}
\bibitem{Wozar:2011gu}
C.~Wozar and A.~Wipf,
\emph{Supersymmetry breaking in low dimensional models,}
Annals Phys. \textbf{327}, 774-807 (2012)
doi:10.1016/j.aop.2011.11.015
[arXiv:1107.3324 [hep-lat]].
%41 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Sakai:2018xkx}
\bibitem{Sakai:2018xkx}
R.~Sakai, D.~Kadoh, Y.~Kuramashi, Y.~Nakamura, S.~Takeda and Y.~Yoshimura,
\emph{Tensor network study of two dimensional lattice $\phi^4$ theory,}
PoS \textbf{LATTICE2018}, 232 (2018)
doi:10.22323/1.334.0232
[arXiv:1812.00166 [hep-lat]].
%1 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Milton:2003av}
\bibitem{Milton:2003av}
K.~A.~Milton,
\emph{PT symmetric quantum field theory,}
Czech. J. Phys. \textbf{53}, 1069-1072 (2003)
doi:10.1023/B:CJOP.0000010535.56276.7e
[arXiv:hep-th/0308033 [hep-th]].
%0 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Joseph:2020gdh}
\bibitem{Joseph:2020gdh}
A.~Joseph and A.~Kumar,
\emph{Complex Langevin dynamics and supersymmetric quantum mechanics,}
JHEP \textbf{10} (2021), 186
doi:10.1007/JHEP10(2021)186
[arXiv:2011.08107 [hep-lat]].
%2 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Joseph:2019sof}
\bibitem{Joseph:2019sof}
A.~Joseph and A.~Kumar,
\emph{Complex Langevin Simulations of Zero-dimensional Supersymmetric Quantum Field Theories,}
Phys. Rev. D \textbf{100} (2019), 074507
doi:10.1103/PhysRevD.100.074507
[arXiv:1908.04153 [hep-th]].
%10 citations counted in INSPIRE as of 26 Jan 2022


%\cite{Golterman:1988ta}
\bibitem{Golterman:1988ta}
M.~F.~L.~Golterman and D.~N.~Petcher,
\emph{A local interactive lattice model with supersymmetry,}
Nucl. Phys. B \textbf{319}, 307-341 (1989)
doi:10.1016/0550-3213(89)90080-1
%70 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Catterall:2003ae}
\bibitem{Catterall:2003ae}
S.~Catterall and S.~Karamov,
\emph{A lattice study of the two-dimensional Wess-Zumino model,}
Phys. Rev. D \textbf{68}, 014503 (2003)
doi:10.1103/PhysRevD.68.014503
[arXiv:hep-lat/0305002 [hep-lat]].
%61 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Baumgartner:2011jw}
\bibitem{Baumgartner:2011jw}
D.~Baumgartner, K.~Steinhauer and U.~Wenger,
\emph{Supersymmetry breaking on the lattice: the $N = 1$ Wess-Zumino model,}
PoS \textbf{LATTICE2011}, 253 (2011)
doi:10.22323/1.139.0253
[arXiv:1111.6042 [hep-lat]].
%12 citations counted in INSPIRE as of 26 Jan 2022

%\cite{Nagata:2016vkn}
\bibitem{Nagata:2016vkn}
K.~Nagata, J.~Nishimura and S.~Shimasaki,
\emph{Argument for justification of the complex Langevin method and the condition for correct convergence,}
Phys. Rev. D \textbf{94}, no.11, 114515 (2016)
doi:10.1103/PhysRevD.94.114515
[arXiv:1606.07627 [hep-lat]].
%99 citations counted in INSPIRE as of 26 Jan 2022



%%%%
%IKKT model 

\bibitem{Ishibashi:1996xs}
N.~Ishibashi, H.~Kawai, Y.~Kitazawa and A.~Tsuchiya, \emph{{A Large N reduced
		model as superstring}},
\href{https://doi.org/10.1016/S0550-3213(97)00290-3}{\emph{Nucl. Phys. B}
	{\bfseries 498} (1997) 467}
[\href{https://arxiv.org/abs/hep-th/9612115}{{\ttfamily hep-th/9612115}}].

\bibitem{Green:1983wt}
M.B.~Green and J.H.~Schwarz, \emph{{Covariant Description of Superstrings}},
\href{https://doi.org/10.1016/0370-2693(84)92021-5}{\emph{Phys. Lett. B}
	{\bfseries 136} (1984) 367}.

\bibitem{Klauder:1983nn}
J.R.~Klauder, \emph{{Stochastic quantization}},
\href{https://doi.org/10.1007/978-3-7091-7651-1_8}{\emph{Acta Phys. Austriaca
		Suppl.} {\bfseries 25} (1983) 251}.

\bibitem{Parisi:1984cs}
G.~Parisi, \emph{{On complex probabilities}},
\href{https://doi.org/10.1016/0370-2693(83)90525-7}{\emph{Phys. Lett.}
	{\bfseries 131B} (1983) 393}.

\bibitem{Krauth:1998xh}
W.~Krauth, H.~Nicolai and M.~Staudacher, \emph{{Monte Carlo approach to M
		theory}}, \href{https://doi.org/10.1016/S0370-2693(98)00557-7}{\emph{Phys.
		Lett. B} {\bfseries 431} (1998) 31}
[\href{https://arxiv.org/abs/hep-th/9803117}{{\ttfamily hep-th/9803117}}].

\bibitem{Austing:2001pk}
P.~Austing and J.F.~Wheater, \emph{{Convergent Yang-Mills matrix theories}},
\href{https://doi.org/10.1088/1126-6708/2001/04/019}{\emph{JHEP} {\bfseries
		04} (2001) 019} [\href{https://arxiv.org/abs/hep-th/0103159}{{\ttfamily
		hep-th/0103159}}].

\bibitem{Hotta:1998en}
T.~Hotta, J.~Nishimura and A.~Tsuchiya, \emph{{Dynamical aspects of large N
		reduced models}},
\href{https://doi.org/10.1016/S0550-3213(99)00056-5}{\emph{Nucl. Phys. B}
	{\bfseries 545} (1999) 543}
[\href{https://arxiv.org/abs/hep-th/9811220}{{\ttfamily hep-th/9811220}}].

\bibitem{Ambjorn:2000dx}
J.~Ambjorn, K.N.~Anagnostopoulos, W.~Bietenholz, T.~Hotta and J.~Nishimura,
\emph{{Monte Carlo studies of the IIB matrix model at large N}},
\href{https://doi.org/10.1088/1126-6708/2000/07/011}{\emph{JHEP} {\bfseries
		07} (2000) 011} [\href{https://arxiv.org/abs/hep-th/0005147}{{\ttfamily
		hep-th/0005147}}].

\bibitem{Anagnostopoulos:2012ib}
K.N.~Anagnostopoulos, T.~Azuma and J.~Nishimura, \emph{{Monte Carlo Simulations
		of a Supersymmetric Matrix Model of Dynamical Compactification in Non
		Perturbative String Theory}},
\href{https://doi.org/10.22323/1.164.0226}{\emph{PoS} {\bfseries LATTICE2012}
	(2012) 226} [\href{https://arxiv.org/abs/1211.0950}{{\ttfamily 1211.0950}}].

\bibitem{Seiler:2012wz}
E.~Seiler, D.~Sexty and I.-O.~Stamatescu, \emph{{Gauge cooling in complex
		Langevin for QCD with heavy quarks}},
\href{https://doi.org/10.1016/j.physletb.2013.04.062}{\emph{Phys. Lett. B}
	{\bfseries 723} (2013) 213}
[\href{https://arxiv.org/abs/1211.3709}{{\ttfamily 1211.3709}}].

\bibitem{Nagata:2016vkn}
K.~Nagata, J.~Nishimura and S.~Shimasaki, \emph{{Argument for justification of
		the complex Langevin method and the condition for correct convergence}},
\href{https://doi.org/10.1103/PhysRevD.94.114515}{\emph{Phys. Rev. D}
	{\bfseries 94} (2016) 114515}
[\href{https://arxiv.org/abs/1606.07627}{{\ttfamily 1606.07627}}].

\bibitem{Ito:2016efb}
Y.~Ito and J.~Nishimura, \emph{{The complex Langevin analysis of spontaneous
		symmetry breaking induced by complex fermion determinant}},
\href{https://doi.org/10.1007/JHEP12(2016)009}{\emph{JHEP} {\bfseries 12}
	(2016) 009} [\href{https://arxiv.org/abs/1609.04501}{{\ttfamily
		1609.04501}}].

\bibitem{Wetterich:1982eh}
C.~Wetterich, \emph{{Massless Spinors in More Than Four-dimensions}},
\href{https://doi.org/10.1016/0550-3213(83)90191-8}{\emph{Nucl. Phys. B}
	{\bfseries 211} (1983) 177}.

\bibitem{Anagnostopoulos:2020xai}
K.N.~Anagnostopoulos, T.~Azuma, Y.~Ito, J.~Nishimura, T.~Okubo and
S.~Kovalkov~Papadoudis, \emph{{Complex Langevin analysis of the spontaneous
		breaking of 10D rotational symmetry in the Euclidean IKKT matrix model}},
\href{https://doi.org/10.1007/JHEP06(2020)069}{\emph{JHEP} {\bfseries 06}
	(2020) 069} [\href{https://arxiv.org/abs/2002.07410}{{\ttfamily
		2002.07410}}].

\bibitem{Nishimura:2011xy}
J.~Nishimura, T.~Okubo and F.~Sugino, \emph{{Systematic study of the SO(10)
		symmetry breaking vacua in the matrix model for type IIB superstrings}},
\href{https://doi.org/10.1007/JHEP10(2011)135}{\emph{JHEP} {\bfseries 10}
	(2011) 135} [\href{https://arxiv.org/abs/1108.1293}{{\ttfamily 1108.1293}}].

\bibitem{Bonelli:2002mb}
G.~Bonelli, \emph{{Matrix strings in pp wave backgrounds from deformed
		superYang-Mills theory}},
\href{https://doi.org/10.1088/1126-6708/2002/08/022}{\emph{JHEP} {\bfseries
		08} (2002) 022} [\href{https://arxiv.org/abs/hep-th/0205213}{{\ttfamily
		hep-th/0205213}}].


\end{thebibliography}

